Towards Assessing and Benchmarking Risk-Return Tradeoff of Off-Policy Evaluation

Off-Policy Evaluation (OPE) aims to assess the effectiveness of counterfactual policies using only offline logged data and is often used to identify the top-k promising policies for deployment in online A/B tests. Existing evaluation metrics for OPE estimators primarily focus on the "accuracy" of OPE or that of downstream policy selection, neglecting risk-return tradeoff in the subsequent online policy deployment. To address this issue, we draw inspiration from portfolio evaluation in finance and develop a new metric, called SharpeRatio@k, which measures the risk-return tradeoff of policy portfolios formed by an OPE estimator under varying online evaluation budgets (k). We validate our metric in two example scenarios, demonstrating its ability to effectively distinguish between low-risk and high-risk estimators and to accurately identify the most efficient one. Efficiency of an estimator is characterized by its capability to form the most advantageous policy portfolios, maximizing returns while minimizing risks during online deployment, a nuance that existing metrics typically overlook. To facilitate a quick, accurate, and consistent evaluation of OPE via SharpeRatio@k, we have also integrated this metric into an open-source software, SCOPE-RL (https://github.com/hakuhodo-technologies/scope-rl). Employing SharpeRatio@k and SCOPE-RL, we conduct comprehensive benchmarking experiments on various estimators and RL tasks, focusing on their risk-return tradeoff. These experiments offer several interesting directions and suggestions for future OPE research.

==> checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \textbf{[Yes]}
    % \answerTODO{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \textbf{[No]}
  \item Did you discuss any potential negative societal impacts of your work?
    \textbf{[N/A]}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \textbf{[Yes]}
    % \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
  \textbf{[N/A]}
    % \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \textbf{[N/A]}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{}
    \textbf{[Yes]}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  \textbf{[Yes]}
    % \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
 \textbf{[Yes]}
    % \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \textbf{[Yes]}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerTODO{}
    \textbf{[Yes]}
  \item Did you mention the license of the assets?
    % \answerTODO{}
    \textbf{[Yes]}
  \item Did you include any new assets either in the supplemental material or as a URL?
    % \answerTODO{}
    \textbf{[Yes]}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    % \answerTODO{}
    \textbf{[N/A]}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerTODO{}
    \textbf{[N/A]}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    % \answerTODO{}
    \textbf{[N/A]}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    % \answerTODO{}
    \textbf{[N/A]}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    % \answerTODO{}
    \textbf{[N/A]}
\end{enumerate}

\end{enumerate}

==> tabs_main_benchmark.tex <==
\begin{figure*}[t]
\begin{minipage}[c]{0.99\hsize}
\centering
\scalebox{0.99}{
\begin{tabular}{c}
\begin{minipage}{0.99\hsize}
    \begin{center}
        \includegraphics[clip, width=0.60\linewidth]{figs/label.png}
        \vspace{-2mm}
    \end{center}
\end{minipage}
\\
\\
\begin{minipage}{0.99\hsize}
    \begin{center}
        \includegraphics[clip, width=1.00\linewidth]{figs/main/benchmark_sharpe_ratio_4.png}
        % \\
        % \includegraphics[clip, width=1.00\linewidth]{figs/benchmark_sharpe_ratio_7.png}
        \vspace{-3mm}
        % \caption{Benchmark results with (Top) SharpeRatio@4 and (Bottom) SharpeRatio@7.}
        \caption{Benchmark results with \textbf{SharpeRatio@4}. The star ($\star$) indicates the best estimator(s).}
        \label{fig:sharpe_ratio_benchmark}
    \end{center}
\end{minipage}
\\
\\
\end{tabular}
}
\end{minipage}
\vspace{-6mm}
\end{figure*}
